Causal Strategic Classification: A Tale of Two Shifts

When users can benefit from certain predictive outcomes, they may be prone to act to achieve those outcome, e.g., by strategically modifying their features. The goal in strategic classification is therefore to train predictive models that are robust to such behavior. However, the conventional framework assumes that changing features does not change actual outcomes, which depicts users as "gaming" the system. Here we remove this assumption, and study learning in a causal strategic setting where true outcomes do change. Focusing on accuracy as our primary objective, we show how strategic behavior and causal effects underlie two complementing forms of distribution shift. We characterize these shifts, and propose a learning algorithm that balances between these two forces and over time, and permits end-to-end training. Experiments on synthetic and semi-synthetic data demonstrate the utility of our approach.

==> analysis.bkp.tex <==
\section{Analysis}

\green{
1. $x_r$ only \\
2. most general - $x_c,x_r,u$, gives $\nu_f(u;x')$ \\
3. if using only $x_c$ (and not $x_r$) and $x_c$ indep. $u$, get cov shift \\
4. tradeoff: assuming $x_r$ corr. with $u$, using $x_r$ more also distorts cov shift more.
}

To learn well in causal strategic settings, we must first
understand how strategic behavior and causal effects translate into shifts in the data distribution.
In this section we characterize such shifts
by analyzing the induced marginal $p^f(x^f)$ and conditional $p^f(y^f|x)$,
focusing initially on the two extremes of fully-correlative ($x=x_r$) 
and fully-causal ($x=x_c$) settings, and then proceeding to discuss the more general mixed setting ($x=(x_c,x_r)$).
Note that choosing which features to use---and hence, of what type (when known)---remains at the discretion of the learner.
\looseness=-1

% goal - understand relations between variables: who changes when and how and in response to what

% In essence, as a learning problem, strategic classification is a problem of learning under \emph{distribution shift}, in which the train and test distributions differ.
% Thus, the key to successful learning lies in understanding exactly what type of distribution shift is caused by strategic behavior.
% The goal of our analysis is to shed light on how the structural difference in features---causal vs. correlative---translates into different forms of distribution shift.
% For this end, we analyze the extreme cases of only using $x_{r}$ and only using $x_c$, which provide our main building blocks.
% Learning can then be interpreted as aiming to find the optimal `blend' between using $x_c$ and $x_r$.
% \begin{itemize}
%      \item Strategic classification is a problem of learning under distribution shift.
%      \item The goal of our analysis is to shed light on how the structural difference in features—causal vs. correlative—translates into different forms of distribution shift
%      \item We analyze the extreme cases of only using $x_{r}$ and only using $x_c$, which provide our main building blocks.
%      \item Learning can then be interpreted as aiming to find the optimal `blend' between using $x_c$ and $x_r$.
% \end{itemize}

Throughout we use capital letters to denote random variables (e.g., $X,U,Y$) and lowercase for their realizations (e.g., $x,u,y$).
For simplicity here we present results for deterministic $h^*$,
but these also hold in the stochastic case;
see technical proofs in Appendix \toref.
\todo{[GUY] prove stochastic case in appendix; rewrite sentence}
Our analysis makes use of an `inverse' response mapping operator:
\begin{equation}
\Delta_{f}^{\minus 1}(x') \triangleq \{x \mid \Delta_{f}(x)=x'\}
\end{equation}
which for any `shifted' point $x'$ returns the set of points $x$ from which $x'$ could have originated, and in response to $f$.

% \todo{[GUY] add all proofs to appendix}

% \paragraph{Notation.}
% We use capital letters to denote random variables (e.g., $X,U,Y$) and lowercase for their realizations (e.g., $x,u,y$).
% We denote $p$ as the probability density of the variables from the base distribution of the data (before strategic movement) and $p^f$ as the induced (by $f$) distribution, i.e. the probability density of the variables after the movement as a response to classifier $f$.
% Our analysis relies heavily on the `inverse' response mapping,
% \[
% \Delta_{f}^{\minus 1}(x') \triangleq \{x \,|\, \Delta_{f}(x)=x'\}
% \]
% which defines for any point $x'$ the set of points $x$ which move to $x'$ in response to $f$.

\subsection{Case \#1: Correlative-only features}
Using $x_{r}$ to predict $y$ can be useful due to its correlation with $u$, which is a direct (and potentially distinct) cause of $y$.
When $f$ relies only on $x_{r}$, all of the features that are used for learning are non-causal, hence changes in $x$ do not affect $y$.\looseness=-1
\begin{observation} \label{obs:using only x_r}
When using only $x_{r}$, causal strategic classification reduces to standard strategic classification.
\end{observation}
Denote $x_{r}'=\Delta_{f}(x_{r})$.
% For a classifier $f$,
Our first result shows the connection between
the original and induced distributions.\looseness=-1
% induced marginal $p^f(x'_{r})$ and conditional $p^f(y|x'_{r})$,
% and the base marginal $p(x_{r})$ and conditional $p(y|x_{r})$.
% Namely, it can be shown that:
\begin{lemma}
\label{lem:only_xr}
Let $p(x_r,y)$ be some base distribution.
Then for any classifier $f$, the induced $p^f(x'_r,y)$
can be expressed using the base
marginal $p(x_{r})$ and conditional $p(y|x_{r})$ as:\looseness=-1
% Then for any classifier $f$,
% the induced marginal and conditional are:
\begin{align}
p^f(x_{r}') &=
\int_{x_{r} \in \Delta_{f}^{\minus 1}(x_{r}')}p(x_{r}) \d x_r
\label{eq:only_xr_marginal} \\
\intertext{and}
% p^f(y|x_{r}') =\frac{1}{p^f(x_{r}')} \int_{x_{r} \in \Delta_{f}^{\minus 1}(x_{r}')}p(x_{r})p(y|x_{r}) \d x_r
p^f(y|x_{r}') &=
\int_{x_{r} \in \Delta_{f}^{\minus 1}(x_{r}')}
\frac{p(x_{r})}{p^f(x_{r}')} p(y|x_{r}) \d x_r
\label{eq:only_xr_conditional}
\end{align}
% where $p(x_{r})$ and $p(y|x_{r})$ are the base marginal and conditional distributions, respectively.
\end{lemma}
% \guy{for this and for all of the other mathematical results, add the full calculations to the appendix?}
Eq. \eqref{eq:only_xr_marginal} simply states that the probability of observing some modified $x'_r$ derives from all points $x_r$ that map to it via $\Delta_f$.
Eq. \eqref{eq:only_xr_conditional} then shows that predicting for $x'_r$ its corresponding $y$ (which remains unmodified) requires reasoning about the possible labels of all points in $\Delta^{\minus 1}_f(x'_r)$;
since this is a set, the implication is inherent (informational) uncertainty in $y$,
which cannot be reduced through statistical means (i.e., observing more data from $p^f$).
This reveals the mechanism through which strategic behavior can harm accuracy.
Here, the ratio $\frac{p(x_{r})}{p^f(x_{r}')}$ expresses the degree to which strategic behavior `distorts' the base probability $p(y|x_{r})$
(which already includes any uncertainty due to $u$, and to $x_c$ if it exists).

Overall, Lemma \ref{lem:only_xr} shows that learning when all used features are correlative is susceptible to \emph{full distribution shift}, in which 
both $p(x)$ and $p(y|x)$ can vary.
However, it does provide a useful insight,
which is immediate from Eq. \eqref{eq:only_xr_conditional}:
\begin{corollary} \label{cor:using only x_r}
When using only $x_{r}$,
knowing the base distribution suffices for constructing
the Bayes-optimal classifier.
% samples from the base distribution suffice for learning an optimal classifier.
\end{corollary}
Practically, Cor. \ref{cor:using only x_r} not only reassures us that robust learning
is possible using clean samples,
but also suggests that learning might benefit from incorporating a marginal density estimator, $\phat(x)$, into the training procedure---a notion which we make use of in our proposed algorithm in Sec. \toref.\looseness=-1

% \todo{consider moving to case 3}
% Together, these results shed light on the pros and cons of using only $x_r$.
% On the one hand, since learning reduces to standard strategic classification,
% the classifier is exposed to strategic behavior that is ``pure gaming'',
% which can be detrimental.
% However, since $y$ does not change, learning can exploit the original unmodified data to its full extent---which is beneficial,
% but also means that additional data gathered over time is unlikely to be useful, and hence of limited use.\looseness=-1


% ratio p(x)/p'(x') - 'distortion' of mass
% u contributes uncertainty via p(y|x) only, and so does not appear ditinctly in p'(y'|x)

% eq simply states that p(x') is sum of all x that it could come from
% eq shows that y since y relates on the original x, for x', must account for all possible x - inherent uncertainty
% toghether, full dist shift
% main message is that bayes optimal classifier needs only base dist info

% Hence, when using only $x_{r}$, the induced distribution $p^f$ is constructed entirely from the probabilities $p(x_{r}), p(y|x_{r})$ from the base distribution;
% Eqs. \eqref{eq:only_xr_marginal} and \eqref{eq:only_xr_conditional} reveal the precise form of distribution shift that strategic behavior induces.
% This indicates that in order to find a classifier $f$ which is optimal over $p^f$, we can use samples only from $p$.
% \begin{corollary} \label{cor:using only x_r}
% When using only $x_{r}$, samples from the base distribution
% suffice for learning an optimal classifier.
% \end{corollary}
% Together, Obs. \ref{obs:using only x_r} and Cor. \ref{cor:using only x_r} characterize the pros and cons of using only $x_{r}$.
% Since learning is reduced to standard strategic classification, using only $x_r$ exposes the classifier to strategic behavior that is ``pure gaming''; the result of which is that the best possible accuracy is likely lower (relative to a non-strategic setting). \guy{I'm not sure that the last sentence is true anymore (for norm cost): we saw (on your whiteboard) that for norm cost, in the strategic setting we can get the original optimal accuracy by raising the bar}
% However, since $y$ does not change, learning can exploit the original unmodified data to its full extent.
% Hence, despite accumulating additional (modified) data at later rounds, we can expect learning to quickly converge (in terms of rounds) to the optimal accuracy attainable under strategic behavior.
% \begin{itemize}
    % \item Using $x_{r}$ to predict $y$ can be useful due to its correlation with $u$, which is a direct cause of $y$. When using only $x_{r}$ for prediction, changes in $x$ will not affect $y$.
    % \item \begin{observation} \label{obs:using only x_r}
    %     When using only $x_{r}$, causal strategic classification reduces to standard strategic classification.
    % \end{observation}
    % \item show results for $p^f(x_{r}')$ and $p^f(y|x_{r}')$.
%     \item When using only $x_{r}$, the induced distribution $p^f$ is constructed entirely from the probabilities $p(x_{r}), p(y|x_{r})$ from the base distribution.
%     \item This indicates that in order to find a classifier $f$ which is optimal over $p^f$, we can use samples only from $p$.
%     \item \begin{corollary} 
% When using only $x_{r}$, samples from the base distribution
% suffice for learning an optimal classifier.
% \end{corollary}
% \item The cons of using only $x_r$ are that changes are pure gaming, hence the best possible accuracy is likely lower.
% \item The pros are that since $y$ does not change, learning can exploit the original unmodified data to its full extent, and we can expect learning to converge in a single round to the optimal accuracy attainable under strategic behavior.
% \end{itemize}

\subsection{Case \#2: Causal-only features}
Using $x_{c}$ is useful for learning as it is a direct cause of $y$ in itself.
We now analyze the case of using only $x_c$ for prediction,
which requires us to directly account for $u$.
\paragraph{Independent case.}
We start with the simpler case in which $X_c$ and $U$ are independent. In this case, the base conditional has the following form:
\begin{align}
\label{eq:base_conditional}
p(y|x_c) 
&= \int_{u}p(u|x_c)p(y|x_c, u) \d u \nonumber \\
&= \int_{u}p(u)\cdot \mathbbm{1}{\{y= h^*(x_c, u) \}} \d u \nonumber \\
&= \int_{u:\:y= h^*(x_c, u)}p(u) \d u
\end{align}
which is simply the uncertainty in $y$ due to $u$.
For our next result,
denote $x_{c}'=\Delta_{f}(x_{c})$ and $y'=h^*(x_{c}', u)$.
\begin{lemma}
\label{lem:only_xc}
Let $p(x_c,y)$ be some base distribution,
and assume $x_c{\perp}u$.
Then for any classifier $f$, we have:
\begin{align}
p^f(x_{c}') &= \int_{x_c \in \Delta_{f}^{\minus 1}(x_c')}p(x_c)\d x_c
\label{eq:only_xc_marginal} \\
\intertext{and}
p^f(y'|x_c') 
&= \int_{u}p(u|x_c')p^f(y'|x_c', u) \d u \nonumber \\
&= \int_{u}p(u)\cdot \mathbbm{1}{\{y'= h^*(x_c', u) \}} \d u \nonumber \\
&= \int_{u:\:y'= h^*(x_c', u)}p(u) \d u
\label{eq:only_xc_conditional}
\end{align}
\end{lemma}
\guy{maybe we will keep only the last line of the equation above to save space?}As expected, Eq.~\eqref{eq:only_xc_marginal} shows that the marginal $p^f(x'_c)$ changes in the $x_c$-only case just as in the $x_r$-only case (Eq.~\eqref{eq:only_xr_marginal}),
since the same type of strategic behavior applies to both.
However, for the conditional term, %in which $y'$ \emph{does} change,
Eq.~\eqref{eq:only_xc_conditional} states that the induced $p^f(y'|x'_c)$
is \emph{exactly the same} as the original base $p(y|x)$ (Eq.~\eqref{eq:base_conditional}).
In other words,
we get that for \emph{any} $f$,
it holds that $P(Y'=y'|X_{c}'=x_{c}')=P(Y=y'|X_{c}=x_{c}')$,
which is a special case of \emph{covariate shift} \cite{shimodaira2000improving}.
%\looseness=-1
% p(y|x) is uncertainty in y from unobs u - u is just noise
% eq 9 = eq 11; does *not* depend on f
\todo{rethink what we're trying to say here; use term `decision-dependent cov shift'?}
\begin{corollary} \label{cor:using only x_c when x,u independent}
If $x_c$ and $u$ are independent, then irrespective of $f$, using only $x_{c}$ reduces to learning under covariate shift.
\end{corollary}
% \todo{consider moving to case 3}
% Learning using $x_c$ alone also has pros and cons.
% On the one hand, Cor. \ref{cor:using only x_c when x,u independent} implies that causal effects `cancel out' the uncertainty in $y$ due to strategic behavior;
% for a given $x_{c}'$, predicting $y'$ does \emph{not} require reasoning about possible downstream effects of $f$. %, and marginal information regarding $p(u)$ suffices.
% Nonetheless, deploying $f$ does change the marginal $p^f(x_{c}')$;
% if $f$ incentivizes points to move to low-density regions of $p(x)$
% (i.e., out-of-distribution),
% % if this causes $p^f$ to concentrate mass in areas of low density under $p$
% % (i.e., if points $x'$ move to regoins beyond $p(x)$),
% then data from the base distribution may \emph{not} suffice for robust learning, since may not be informative of those regions.
% % to learn using only data from the base distribution, since $f$ may cause the induced $p^f$ to concentrate mass in areas of low density under $p$.
% This has a dual effect:
% at each round, if $p^f$ concentrates on under-explored regions of $\X$, then we can expect degraded performance \emph{along the way};
% but over time, we can expect induced distributions to collectively cover larger areas of $\X$, which is likely to improve performance \emph{in the long run}.
% Note that here strategic behavior is no longer `gaming';
% rather, it can serve the system as a mechanism of (indirect) exploration that \emph{enables} performance to improve over time.

% Whether data from multiple induced distributions is helpful or not is case-specific, i.e., depends on the $p$ and $h^8$

% over time is essential to learn under covariate shift depends on the distribution and $h^*$; in some cases, it could suffice to use samples from a single distribution \tocite{}.

% ---and in some cases, due to causal effects, might even approach or surpass performance in the non-strategic setting.




% \begin{itemize}
    % \item show results for $p(y|x_c)$, $p^f(x_{c}')$, and $p^f(y'|x_c')$.
    % \item \begin{corollary} \label{cor:using only x_c when x,u independent}
    % If $x_c,u$ are independent, then using only $x_{c}$ reduces to learning under \emph{covariate shift} \cite{shimodaira2000improving}.
    % \end{corollary}
    % \item On one hand, predicting $y'$ does \emph{not} require information regarding $f$ (or $p^f$)
    % \item On the other hand, because $f$ affects the marginal distribution $p^f(x_{c}')$, it may \emph{not} suffice to learn using only data from the base distribution.
    % \item This has a dual effect: over time, we can expect induced distributions to collectively cover larger areas of $\X$, which is likely to improve performance \emph{in the long run}; however, at each time step, if $p^f$ concentrates on under-explored regions of $\X$, then we can expect degraded performance \emph{along the way}.
    % \item here strategic behavior is no longer `gaming'; rather, it serves as a mechanism of (indirect) exploration that \emph{enables} performance to improve---and in some cases, might even approach the non-strategic baseline (using $x_c$)
%     \item \nir{here we can say that under cov shift, sometimes one sample from one distribution suffices for being accurate on other distributions (cite papers) -- and sometimes not. this would hedge off expectations that time is always important, and would make any results we have in which one round suffices be ok.}
% \end{itemize}
\paragraph{Dependent case.}
We now consider the more general case when $x_c$ and $u$ are not independent.
% we get a more complicated expression for $p^f(y'|x_c')$:
% \begin{equation}
% \begin{aligned}
%     & p^f(y'|x_c') = \\
%     & \frac{1}{p^f(x_{c}')}\int_{x_{c} \in \Delta_{f}^{\minus 1}(x_{c}')}\int_{u:\:y'= h^*(x_{c}', u)}p(x_{c}, u) \d u \d x_c
% \end{aligned}
% \end{equation}
\begin{lemma}
For any $p(x'_c,u)$ and any classifier $f$, we have:
\label{lem:only_xc_dep}
\begin{align}
    & p^f(y'|x_c') = 
    \int_{u:\:y'= h^*(x'_{c}, u)}
    \nu_f(u;x'_c) p(u) \d u \label{eq:only_xc_dep_conditional} \\
    \intertext{where:}
    & \nu_f(u;x'_c) = 
    \int_{x_{c} \in \Delta_{f}^{\minus 1}(x_{c}')}
    \frac{p(x_{c} | u)}{p^f(x_{c}')} \d x_c \label{eq:only_xc_dep_nu}
\end{align}
and the marginal $p^f(x'_c)$ is as in Eq. \eqref{eq:only_xc_marginal}.
\end{lemma}
While covariate shift no longer holds,
note that Eq.~\eqref{eq:only_xc_dep_conditional} matches
Eq.~\eqref{eq:only_xc_conditional} up to the term $\nu_f$.
Hence, $\nu_f$ can be thought of as determining how much 
learning deviates from covariate shift as a result of using $f$:
when $\nu_f(u;x_c')$ takes values close to one across $u$,
then covariate shift `approximately' holds;
otherwise, we have a particular form of full distribution shift.
Note that in itself, $\nu_f$ relates to Eq.~\eqref{eq:only_xr_conditional},
in that the strategic effects also express as a distorted probability term integrated over the inverse response set.

% nu is how this deviates from cov shift (close to 1 is more like cov shift)

\todo{think if can connect this to bound on generalization error}

% Here, since $p^f(y'|x_c')$ depends on $f$ and on $p^f(x_{c}')$, this no longer results in covariate shift, but rather a more general form of distribution shift.
% In this case, we are still likely to benefit from additional modified data over time, but must also account for the role $f$ itself plays in determining $p^f(y'|x'_c)$.
% \begin{itemize}
%     \item When $x_c$ and $u$ are not independent, we get a more complicated expression for $p^f(y'|x_c')$
%     \item Show expression
%     \item Here, since $p^f(y'|x_c')$ depends on $f$ and on $p^f(x_{c}')$, this no longer results in covariate shift, but rather a more general form of distribution shift.
%     \item In this case we are still likely to benefit from additional modified data over time, but must also account for the role $f$ itself plays in determining $p^f(y'|x'_c)$.
% \end{itemize}

\subsection{Case \#3: Using all features}\label{sec:analysis_using_all}
Committing to just one feature type is likely sub-optimal;
for example, Eq.~\eqref{eq:only_xc_conditional} shows how $x_r$,
which is informative of $u$, can help reduce uncertainty in $y$
for any given $x_c$.
But since each feature type brings forth different pros and cons,
learning should aim to correctly balance between them. %, as they express over time.

Our analysis thus far demonstrates how each feature type makes
learning susceptible to a different form of distribution shift---full strategic shift (for $x_r$) vs. `approximate' covariate shift (for $x_c$, as it depends on $u$).
When considering these effects over time, we see two complementing forces at play: %\looseness=-1
Correlative features are prone to negative gaming effects,
which can lead to the best attainable accuracy being low;
however, learning should quickly reach this optimal point
since clean data suffices for reducing uncertainty in $y$.
Contrarily, causal features affect $y$; hence, if points move to unexplored territory, then this can hurt performance.
But as dirty data amounts over time and under different $f$,
more out-of-distribution information about $h^*$ is revealed,
which can be used in learning to improve accuracy.
% in effect by negating---or even harnessing---strategic effects.
But even if \emph{eventual} performance can improve,
\emph{along the way} it may deteriorate.\looseness=-1

Thus, fully utilizing both requires learning to account for how they trade off:
$x_r$ offers the quick and sure road to (possibly) lower performance,
whereas $x_c$ offers the long road having higher potential
but costly in time and uncertainty.
We now proceed to present our approach,
which builds on the above conclusions to account for this temporal tradeoff.

% \todo{maybe add to appendix analysis for mixed case}

%===============
% Our analysis regarding using either all-correlative or all-causal features reveals the pros and cons of each feature type.
% When using only $x_r$,
% % On the one hand, since
% learning reduces to standard strategic classification,
% and so the classifier is exposed to strategic behavior that is ``pure gaming'',
% which can be detrimental.
% However, since $y$ does not change, learning can exploit the original unmodified data to its full extent---which is beneficial,
% but also means that additional data gathered over time is unlikely to be useful, and hence of limited use. %\looseness=-1

% Contrarily, when using only $x_c$, 
% % Learning using $x_c$ alone also has pros and cons.
% % On the one hand,
% Cor. \ref{cor:using only x_c when x,u independent} implies that causal effects `cancel out' the uncertainty in $y$ due to strategic behavior;
% for a given $x_{c}'$, predicting $y'$ does \emph{not} require reasoning about possible downstream effects of $f$. %, and marginal information regarding $p(u)$ suffices.
% Nonetheless, deploying $f$ does change the marginal $p^f(x_{c}')$:
% if $f$ incentivizes points to move to low-density regions of $p(x)$
% (i.e., out-of-distribution),
% % if this causes $p^f$ to concentrate mass in areas of low density under $p$
% % (i.e., if points $x'$ move to regoins beyond $p(x)$),
% then data from the base distribution may \emph{not} suffice for robust learning, since it may not be informative of those regions.
% % to learn using only data from the base distribution, since $f$ may cause the induced $p^f$ to concentrate mass in areas of low density under $p$.
% This has a dual effect:
% at each round, if $p^f$ concentrates on under-explored regions of $\X$, then we can expect degraded performance \emph{along the way};
% but over time, we can expect the varying $p^f$ to collectively cover larger areas of $\X$, which can improve performance \emph{in the long run}.
% Note that here strategic behavior is no longer `gaming';
% rather, it can serve as a mechanism for (indirect) exploration that enables performance to improve over time. %\looseness=-1


% \blue{
% \todo{[GUY] plug in bullets (given text above)}
% Our analysis demonstrates how using either only $x_{r}$ or only $x_{c}$ results in different forms of distribution shift---standard strategic classification (for $x_r$) vs. covariate shift (for $x_u$, assuming independence of $u$).
% When considering these effects over time, we can expect two complementing forms of dynamics.
% Using $x_r$ alone quickly leads to optimal accuracy---but this optimal point is relatively low, due to strategic gaming behavior \guy{again, I think the last part is not true}.
% In contrast, using $x_c$ alone has the potential to reach much higher accuracy by utilizing strategic behavior for `exploration';
% this, however, may take time, with accuracy improving at a slow pace.

% xc case shows u is important - motivates using xr, since it correlates

% Ultimately, this reveals a trade-off between using causal and correlative features for prediction. Recalling that both $x_c$ and $x_r$ are informative of $y$ (and therefore of potential use for prediction),
% and that the \emph{degree} to which they are used in prediction is controlled by the learner (this is easy to see in linear models),
% we come to the conclusion that learning well over time requires the learner to find an optimal balance between $x_c$ and $x_r$, as learning progresses over time.
% As we will see in the next section, this is the core idea underlying our approach.

% \begin{itemize}
%     % \item Using either only $x_{r}$ or only $x_{c}$ results in different forms of distribution shift: standard strategic classification vs. covariate shift
%     % \item Using $x_r$ alone quickly leads to optimal accuracy---but this optimal point could be low, due to strategic gaming behavior.
%     % \item Using $x_c$ alone has the potential to reach much higher accuracy by utilizing strategic behavior for `exploration'; this, however, may take time, with accuracy improving at a slow pace.
%     \item Ultimately, this reveals a trade-off between using causal and correlative features for prediction. Both $x_c$ and $x_r$ are informative of $y$ (and therefore of potential use for prediction), and the \emph{degree} to which they are used in prediction is controlled by the learner, we come to the conclusion that learning well over time requires us to find an optimal balance between $x_c$ and $x_r$, as learning progresses over time. As we will see in the next section, this is the core idea underlying our approach.
% \end{itemize}
% \nir{since we don't have any precise statement here, would be good to think of how we complement this experimentally --- once our basic synthetic setup will be in place, what would be interesting to demonstrate empirically?}
% }

% \blue{
% \begin{itemize}
    % \item Note that while $u$ is unobserved, it is still relevant since labels are drawn from the conditions $y \sim p(y|x_c,x_r,u)$.
    % \item Although $x_r$ are "only" correlative, they are still relevant since $u$ is unobserved, then if $x_r$ is informative of $u$, it can be utilized for predicting y.
    % \item The objective introduces three distinct challenges: (i) $\Delta_f$ is non-differentiable (and even discontinuous) due to the argmax operator, (ii) $u$ is unknown at train time, and (iii) $h^*$ is unknown at train time; the latter two challenges are unique to our causal setting.
    % \item the objective raises issues of statistical gaps, i.e. if we would want to estimate $h^*$ influence on manipulated data we will need collect manipulated samples in addition to the clean samples.
% \end{itemize}

% information gaps:
% \nir{in other words - can't ever have true $h^*(x'_c,u)$ in empirical objective. these gaps cannot be fully reduced (vs statistical gaps, which can - this is not knowing $h^*$)}
% \begin{itemize}
% % \item strategic: we only observe the modified $x'$ -- and while $x'_c$ is informative of $y'$, we do not have the original $x_r$
% \item correlative: $u$ is unobserved -- even if we know $x_r$, we cannot fully recover $u$
% \item causal: original `clean' $x$ is unobserved -- even if we know $\Delta$ and $p(x)$, still $\Delta^{-1}(x')$ is a set, and so we cannot precisely recover $x$
% \nir{more precise: at train time, we don't have $\xtilde = (x'_c,x_r)$, which is what we be best for estimating $\ytilde = h^*(\xtilde)$ -- which is best we can hope for without having $u$}
% \nir{in principle, if $\Delta$ was one-to-one, we could maybe hope to learn $\Delta^{-1}$, and hence would be ok with seeing only $(x_c,x_r)$ or $(x'_c,x'_r)$, because we could hope to learn the inverse mapping $\Delta^{-1}$ (ie, it would be a statistical gap). but our $\Delta$ is lossy, so will always have information gap.}
% \guy{I don't think we can talk about this information gap here. this is relevant to the process of "fixing" dirty samples, and we are introducing this process only in section 5}
% \end{itemize}
% however, we will show how learning can utilize `clean' + temporal `dirty' data to reduce these gaps
% }
